Unlocking the Power of Spatial and Temporal Information in Medical Multimodal Pre-training

Medical vision-language pre-training methods mainly leverage the correspondence between paired medical images and radiological reports. Although multi-view spatial images and temporal sequences of image-report pairs are available in off-the-shelf multi-modal medical datasets, most existing methods have not thoroughly tapped into such extensive supervision signals. In this paper, we introduce the Med-ST framework for fine-grained spatial and temporal modeling to exploit information from multiple spatial views of chest radiographs and temporal historical records. For spatial modeling, Med-ST employs the Mixture of View Expert (MoVE) architecture to integrate different visual features from both frontal and lateral views. To achieve a more comprehensive alignment, Med-ST not only establishes the global alignment between whole images and texts but also introduces modality-weighted local alignment between text tokens and spatial regions of images. For temporal modeling, we propose a novel cross-modal bidirectional cycle consistency objective by forward mapping classification (FMC) and reverse mapping regression (RMR). By perceiving temporal information from simple to complex, Med-ST can learn temporal semantics. Experimental results across four distinct tasks demonstrate the effectiveness of Med-ST, especially in temporal classification tasks. Our code and model are available at https://github.com/SVT-Yang/MedST.

==> tables/seqlength.tex <==

\begin{table*}[t]
\caption{}
\label{tab:seqlength}
\vskip -0.3in
\begin{center}
% \begin{small}
% \begin{sc}
\begin{tabular}{l|ccccc|c}
\toprule



Seq.length         & Consolidation & Edema & Pl.effusion & Pneumonia & Pneumothorax & \textbf{Avg. Acc.}    \\ \midrule

4           & {60.57}\tiny{$\pm$ 1.18}       &{67.35}\tiny{$\pm$ 0.32} & {58.47}\tiny{$\pm$ 1.50}         & {65.00\tiny{$\pm$ 0.34}}     & {54.18}\tiny{$\pm$ 0.81}     & {61.12}\tiny{$\pm$ 0.34}\\

6           & {58.89}\tiny{$\pm$ 0.27}       &{63.32}\tiny{$\pm$ 0.46} & {58.72}\tiny{$\pm$ 0.50}         & {66.26\tiny{$\pm$ 0.34}}     & {55.31}\tiny{$\pm$ 0.78}     & {60.50}\tiny{$\pm$ 0.17}

\bottomrule
\end{tabular}
% \end{sc}
% \end{small}
\end{center}
\end{table*}

